Lisco: A Continuous Approach in LiDAR Point-cloud Clustering

The light detection and ranging (LiDAR) technology allows to sense surrounding objects with fine-grained resolution in a large areas. Their data (aka point clouds), generated continuously at very high rates, can provide information to support automated functionality in cyberphysical systems. Clustering of point clouds is a key problem to extract this type of information. Methods for solving the problem in a continuous fashion can facilitate improved processing in e.g. fog architectures, allowing continuous, streaming processing of data close to the sources. We propose Lisco, a single-pass continuous Euclidean-distance-based clustering of LiDAR point clouds, that maximizes the granularity of the data processing pipeline. Besides its algorithmic analysis, we provide a thorough experimental evaluation and highlight its up to 3x improvements and its scalability benefits compared to the baseline, using both real-world datasets as well as synthetic ones to fully explore the worst-cases.

==> sections/frombatchtostream.tex <==
\section{From batch to stream}\label{sec:frombatchtostream}


State of the art clustering of \lidar{} data (e.g. the one provided by the PCL library) operates in a batch fashion. That is, it first waits for one batch of $S$ steps to be delivered, it then clusters them (by applying the removal of the ground, building the tree and finally running Euclidean cluster extraction, as discussed in \autoref{sec:pcl}). When shifting to the streaming model, our goal is to define a clustering algorithm that allows for the set of $L$ points delivered at each step to immediately go through the processing pipeline of ground removal and clustering. In this sense, to ideally complete the analysis of the points at step $x$ before the points from step $x+1$ are delivered, nonetheless, requires fast one-pass analysis of data, as prescribed by the data streaming processing paradigm.

\paragraph{Cluster in space and time} State of the art clustering is based on space clustering only \vincom{References OR SPECULATION}. It is desirable, nonetheless, to extend the expressiveness of clustering to the time dimension too. \vincom{Here maybe we need to say ``if the user wants that"}. We show this in the following example.

In the example, an object moving close to the \lidar{} sensor is first hit by the lasers at rotation step $x=1$. By the time the lasers complete the rotation ($x=S$) the lasers hit the object again. By clustering this over space only, the algorithm might detect and object very big when in practice it is small.

\paragraph{continuous production of results} You think the previous point is a problem? not really if you produce results continuously. Check this thing here...

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{figures/timespaceclustering}
  \caption{XXX.}
  \label{fig:timespaceclustering}
\end{figure}
